HeLM: Highlighted Evidence augmented Language Model for Enhanced Table-to-Text Generation

Large models have demonstrated significant progress across various domains, particularly in tasks related to text generation. In the domain of Table to Text, many Large Language Model (LLM)-based methods currently resort to modifying prompts to invoke public APIs, incurring potential costs and information leaks. With the advent of open-source large models, fine-tuning LLMs has become feasible. In this study, we conducted parameter-efficient fine-tuning on the LLaMA2 model. Distinguishing itself from previous fine-tuning-based table-to-text methods, our approach involves injecting reasoning information into the input by emphasizing table-specific row data. Our model consists of two modules: 1) a table reasoner that identifies relevant row evidence, and 2) a table summarizer that generates sentences based on the highlighted table. To facilitate this, we propose a search strategy to construct reasoning labels for training the table reasoner. On both the FetaQA and QTSumm datasets, our approach achieved state-of-the-art results. Additionally, we observed that highlighting input tables significantly enhances the model's performance and provides valuable interpretability.

==> miscs/figure_prompt_egpt.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=1.0\textwidth]{miscs/prompt_egpt.pdf}
    \caption{The prompt used to obtain $E_{gpt}$ using GPT-3.5-trubo. The content within the green brackets represents two examples used for few-shot learning. The inputs such as tables, queries, etc., within the red brackets, can be replaced according to specific input requirements.}
    \vspace*{0.4cm}
    \label{fig:prompt_egpt}
\end{figure*}
% 这是使用 GPT3.5-trubo 来获得 Egpt 所使用的 prompt。绿色括号里的内容代表来进行 fewshot-learning 的两个例子。红色括号中的输入 table，query 等可根据具体的输入替换。



==> miscs/figure_prompt_example.tex <==
\begin{figure}[hp]
\centering

\includegraphics[width=\linewidth]{miscs/prompt_example1.pdf} \\
\includegraphics[width=\linewidth]{miscs/prompt_example2.pdf}
\caption{Two examples used in figure \ref{fig:prompt_egpt}}
\vspace*{0.4cm}
\label{fig:prompt_example}
\end{figure}



==> miscs/table_fetaqa_aba.tex <==

\begin{table}[h]
  \centering
  \begin{tabular}{lp{7mm}p{7mm}p{7mm}p{8mm}} \toprule
        Models          & R-1  & R-2  & R-L  & BLEU    \\ \midrule
        \multicolumn{5}{c}{Different highlight evidence} \\ \midrule
$\text{LLaMA2-13B}^{\dag}$&  66.5 &  44.7 &  56.2 & 33.24  \\
$\text{HeLM-13B}^{\dag}$&  67.8 &  46.4 &  57.9 & 35.10  \\
         - w/o highlight       &  66.6 &  44.7 &  56.6 & 33.13  \\
         - subTab       &  65.0 &  43.3 &  55.5 & 32.28  \\
- $E_{distill\ w/o\ \mathcal{Y}}$&68.1&  46.6 &  58.1 & 35.34  \\
         - $E_{distill}$    &  69.4 &  47.8 &  59.2 & 36.33  \\
         - $E_{search}$     &  68.1 &  46.6 &  58.0 & 34.96  \\
         - $E_{merge}$  &  69.6 &  48.2 &  59.5 & 36.74  \\  \midrule
         \multicolumn{5}{c}{Different model size} \\ \midrule
$\text{LLaMA2-7B}^{\dag}$&  65.0 &  43.0 &  54.8 & 32.68  \\
$\text{HeLM-7B}^{\dag}$& 65.4 &  43.5 &  55.4 & 32.95  \\
         - w/o highlight       &  64.7 &  43.0 &  54.8 & 32.28  \\ 
         % \multicolumn{5}{c}{Different summarizer} \\ \midrule
         % Summarizer-$\mathcal{M}_S^0$  &  67.6 &  46.1 &  57.6 & 34.93  \\
         \bottomrule
  \end{tabular}
  \caption{Ablation study on FeTaQA dataset. The $\dag$ marked models are trained using QLoRA.} 
  \vspace*{0.4cm}
  \label{tab:aba1}
\end{table}
%带有 * 上标的表示是用 qlora 训练的模型。
